Mitigating Outages in a 4.6-km FSO Link via Mode-Diverse Reception: An Experimentally Validated Digital Twin Approach

Terrestrial coherent FSO requires mitigating turbulence-induced coupling losses. We experimentally validate a "Digital Twin" channel model against fading statistics from a 4.6-km link. Combining long-term scintillometer data with mode-diverse receiver simulations, we demonstrate that a 6-mode receiver reduces turbulence-induced outage probabilities to 2.02e-5.

==> figures/outage/weighted_outage.tex <==
% Recommended preamble:
\begin{tikzpicture}
    \def\datafile{figures/outage/Pout_vs_cn2.csv}
    \def\cnfile{figures/outage/cn2_kde.csv}
    \tikzset{font=\footnotesize}
    \pgfplotsset{compat=1.18}
    \usepgfplotslibrary{fillbetween}
    \begin{axis}[
        width=\linewidth, 
        height=0.6*\axisdefaultheight, 
        axis lines={left}, 
        xlabel={{Refractive Index Structure Constant $C_n^2/\qty{}{m^{-2/3}}$}}, 
        ylabel={{$P_\text{out}(C_{n}^{2}) \cdot p(C_{n}^{2})$}}, 
        enlarge x limits={{rel=0.1, upper}}, 
        enlarge y limits={{rel=0.1, upper}}, 
        xmode=log,
        ymode=log,
        xmin={1.5e-16},
        xmax={1.5e-13},
        ymin={1e-3}, 
        grid, 
        legend columns={-1}, 
        legend style={{ /tikz/every even column/.append style={column sep=0.25cm}, draw = none, at = {(0.5, 1.05)}, anchor = south }}
    ]
        % Baseline for area fill on log-scale y-axis (must be > 0)
        \path[name path=baseline1] (axis cs:3.7678296472643703e-16,1e-3) -- (axis cs:1.5e-13,1e-3);
        \path[name path=baseline2] (axis cs:1.5e-15,1e-3) -- (axis cs:1.5e-13,1e-3);
        \path[name path=baseline3] (axis cs:1.1914923520864222e-14,1e-3) -- (axis cs:1.5e-13,1e-3);

        % Filled areas under curves
        \addplot[name path=smfcurve, draw=none,forget plot] table[col sep=comma, x=x, y=y1p] {\datafile};
        \addplot[okabe_ito_1, draw=none, fill opacity=0.15,forget plot] fill between[of=smfcurve and baseline1];

        \addplot[name path=fmf3curve, draw=none, forget plot] table[col sep=comma, x=x, y=y3p] {\datafile};
        \addplot[okabe_ito_2, draw=none, fill opacity=0.15, forget plot] fill between[of=fmf3curve and baseline2];

        \addplot[name path=fmf6curve, draw=none, forget plot] table[col sep=comma, x=x, y=y6p] {\datafile};
        \addplot[okabe_ito_3, draw=none, fill opacity=0.15, forget plot] fill between[of=fmf6curve and baseline3];

        % Plot 1: SMF
        \addplot[okabe_ito_1,thick, mark=*] table[col sep=comma, x=x, y=y1p] {\datafile};
        % Plot 2: FMF3
        \addplot[okabe_ito_2,thick,mark=x] table[col sep=comma, x=x, y=y3p] {\datafile};
        % Plot 3: FMF6
        \addplot[okabe_ito_3,thick,mark=o] table[col sep=comma, x=x, y=y6p] {\datafile};
        % % Plot 4: p(Cn2)
        % \addplot+[thick] table[col sep=comma, x=cn2, y=pdf] {\cnfile};

        % Legend entries
        \addlegendentry {SMF}; 
        \addlegendentry {FMF3}; 
        \addlegendentry {FMF6}; 

        % Inset with additional information
        \node[draw, fill=white, align=center, anchor=north east] at (rel axis cs:1,1) {\(L_\text{th}=\qty{10}{dB}\)};
    \end{axis}
\end{tikzpicture}%
